Can LLMs reason over extended multilingual contexts? Towards long-context evaluation beyond retrieval and haystacks

Existing multilingual long-context benchmarks, often based on the popular needle-in-a-haystack test, primarily evaluate a model's ability to locate specific information buried within irrelevant texts. However, such a retrieval-centric approach is myopic and inherently limited, as successful recall alone does not indicate a model's capacity to reason over extended contexts. Moreover, these benchmarks are susceptible to data leakage, short-circuiting, and risk making the evaluation a priori identifiable. To address these limitations, we introduce MLRBench, a new synthetic benchmark for multilingual long-context reasoning. Unlike existing benchmarks, MLRBench goes beyond surface-level retrieval by including tasks that assess multi-hop inference, aggregation, and epistemic reasoning. Spanning seven languages, MLRBench is designed to be parallel, resistant to leakage, and scalable to arbitrary context lengths. Our extensive experiments with an open-weight large language model (LLM) reveal a pronounced gap between high- and low-resource languages, particularly for tasks requiring the model to aggregate multiple facts or predict the absence of information. We also find that, in multilingual settings, LLMs effectively utilize less than 30% of their claimed context length. Although off-the-shelf Retrieval Augmented Generation helps alleviate this to a certain extent, it does not solve the long-context problem. We open-source MLRBench to enable future research in improved evaluation and training of multilingual LLMs.

==> figures/distractor_examples.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth,keepaspectratio,trim={0 0 0 0},clip]{latex/figures/distractor_examples.pdf}
\caption{Example of different distractors}
\label{fig:distractor_examples}
% \vspace{-0.5mm}
% \vspace{-5mm}
\end{figure*}

==> figures/line_charts.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{latex/figures/line-charts.pdf}
    \caption{Monolingual long-context performance across different context sizes}

    
\end{figure*}

==> sections/ethics_statement.tex <==
%\paragraph{\bf Ethics Statement}
Our proposed \dataset\ benchmark is completely synthetic.  We have not involved any human annotators while curating \dataset\ . Our work does not need any additional ethical review by an institutional review board. All the models, datasets, and scientific artefacts used in this study have been properly citated wherever required. 

==> sections/interpretation.tex <==
\section{Interpretation}
\prasoon \\

We need to compare performance at 0k vs 64k?

==> sections/plots_and_figures.tex <==
\section{Tables}
\amey

\begin{enumerate}

\item Table1 - Dataset Statistics.

\item Table2 - Main Results. 

\item Table3 - Task-specific results. 

\item Table4 - Statistical Test

\item Figure1 - Generation of multilingual bAbI dataset

    
\end{enumerate}

\section{Plots, and Figures}
\prasoon

\begin{enumerate}
\item Plot1 - Should capture monolingual long-context performance across different context sizes. 





\input{figures/line-lang-avg-method}
\input{figures/line-method-avg-lang}

% \input{figures/radar-lang-across_method-avg_context}
% \input{figures/radar-lengths-across_method-avg_lang}


% \input{figures/line_charts}
% \input{figures/radar_lang}
% \input{figures/radar_lengths}





\item Plot2 - Effect of change in language - across different context sizes. \cite{}

\item Plot3 - RAG vs Long-context. 

\item Plot4 - Ablations



\end{enumerate}

==> tables/dataset.tex <==
% \begin{table}[h]
% \centering
% \begin{tabular}{|>{\hspace{0pt}}m{0.681\linewidth}|>{\hspace{0pt}}m{0.206\linewidth}|}
% Dataset Size               & \$7000\$  \\
% Total Languages            & \$7\$     \\
% Queries per Language       & \$1000\$  \\
% Dev Set Size per Language  & \$500\$   \\
% Test Set Size per Language & \$500\$  \\
% Average Passage Length & \\
% Average facts per passage & \\
% \end{tabular}
% \label{tab:dataset_info}
% \caption{Dataset statistics}
% \end{table}

==> tables/distractor_example_table.tex <==
% \begin{table*}[!t]
% \small
% \begin{center}
% \scalebox{0.9}{
%   \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{
% >{\raggedright\arraybackslash}p{4cm}|
% >{\raggedright\arraybackslash}p{13.5cm}
% }
% \hline
% \textbf{Distractor Type} & \textbf{Example Prompt} \\
% \hline
% Synthetic Distractors & \texttt{<context>} \\ \textbf{Bertha ging ins Badezimmer}. Bertha ist nicht im Badezimmer \textbf{Lukas ging zurück in den Flur}. Die Badezimmer sind in der Regel ein wichtiger Teil eines Hauses... \textbf{Sabine ging zurück ins Büro}. \textbf{Sabine ging zurück in den Flur}. Hans ging zurück ins Badezimmer... \textbf{Lukas ging in die Küche}. \textbf{Hans ging in die K\"uche.Lukas ging ins Schlafzimmer}. \textbf{Sabine ging in die K\"uche}. \textbf{Hans ging ins Schlafzimmer}. \\ \texttt{</context>} \\ \\ Question: Wo ist Hans? \\ Answer: \textcolor{ForestGreen}{Hans ist im Schlafzimmer} \\
% \hline
% Sourced from public dataset (MLQA) & \texttt{<context>} \\ Phoebe war vor Beginn der Serie lange Monicas Mitbewohnerin... \textbf{Bertha ging ins Badezimmer}. Ihr Vater Frank hat die Familie... \textbf{Lukas ging zurück in den Flur}. Sp\"ater erf\"ahrt sie, dass Phoebe Abbott... \textbf{Sabine ging zurück ins Büro}. \textbf{Sabine ging zurück in den Flur}. Hans ging zurück ins Badezimmer... \textbf{Lukas ging in die Küche}. \textbf{Hans ging in die K\"uche.Lukas ging ins Schlafzimmer}. \textbf{Sabine ging in die K\"uche}. \textbf{Hans ging ins Schlafzimmer}. \\ \texttt{</context>} \\ \\ Question: Wo ist Hans? \\ Answer: \textcolor{ForestGreen}{Hans ist im Schlafzimmer} \\
% \hline
% Randomly Generated Distractors & \texttt{<context>} \\ ######################## \textbf{Bertha ging ins Badezimmer}.####################... \textbf{Lukas ging zurück in den Flur}.###########################... \textbf{Sabine ging zurück ins Büro}.###########################... \textbf{Sabine ging zurück in den Flur}.###########################... Hans ging zurück ins Badezimmer... \textbf{Lukas ging in die Küche}. \textbf{Hans ging in die K"uche.Lukas ging ins Schlafzimmer}. \textbf{Sabine ging in die K"uche}. \textbf{Hans ging ins Schlafzimmer}. \\ \texttt{</context>} \\ \\ Question: Wo ist Hans? \\ Answer: \textcolor{ForestGreen}{Hans ist im Schlafzimmer} \\
% \hline
% \end{tabular}}
% \caption{Examples of different distractor types used in context to evaluate model robustness.}
% \label{tab:distractor-examples}
% \end{center}
% \end{table*}

==> tables/prompt_templates.tex <==
% \begin{table*}[!ht]
% \begin{center}
% \small % Reducing the font size
% \setlength{\tabcolsep}{2pt} % Adjusting column separation
% \renewcommand{\arraystretch}{1.0} % Reducing cell padding
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{p{1.3in}p{5.2in}}
% \toprule
% \textbf{\texttt{Prompt Template for Capturing the Action (Moderate-Length Distractor)}} &
%   \begin{tabular}[c]{@{}p{5.2in}@{}}
%   \texttt{You are given an independent sentence from the bAbI dataset, which follows the Subject -> Action -> Object structure.}\\\\
%   \texttt{\#\#\# Sentence}\\
%   \texttt{\{sentence\}}\\\\
%   \texttt{\#\#\# Task}\\
%   \texttt{Generate a story or passage (100-200 words) that captures the essence of the action but never mentions the subject or the object.}\\\\
%   \texttt{\#\#\# Constraints}\\\\
%   \texttt{- The action may appear, but it must be used in a completely different meaning or context than in the original sentence.}\\\\
%   \texttt{- The passage must contain multiple sentences that expand on the topic with background information, examples, or applications.}\\\\
%   \texttt{- The passage must have no semantic or narrative connection to the original sentence.}\\\\
%   \texttt{- The passage must be complex enough to act as a distractor when answering a question about the original sentence.}\\\\
%   \texttt{- The passage could include any topic such as science, sports, economics, politics, medicine, philosophy, history, or technology.}\\\\
%   \texttt{- The passage must be in the same language as the input sentence.}\\\\
%   \texttt{\#\#\# Output}\\
%   \texttt{Strictly output only the distractor passage and nothing else.}
%   \end{tabular} \\
% \bottomrule
% \end{tabular}%
% }
% \end{center}
% \caption{Prompt template used for generating a moderate-length distractor passage by capturing the action but omitting the subject and object.}
% \label{tab:prompt_template_case_1}
% \end{table*}

% \begin{table*}[!ht]
% \begin{center}
% \small
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.0}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{p{1.3in}p{5.2in}}
% \toprule
% \textbf{\texttt{Prompt Template for Including Only the Subject (Moderate-Length Distractor)}} &
%   \begin{tabular}[c]{@{}p{5.2in}@{}}
%   \texttt{You are given an independent sentence from the bAbI dataset, which follows the Subject -> Action -> Object structure.}\\\\
%   \texttt{\#\#\# Sentence}\\
%   \texttt{\{sentence\}}\\\\
%   \texttt{\#\#\# Task}\\
%   \texttt{Generate a moderate-length passage (100-200 words) that includes the subject but never mentions the action or the object.}\\\\
%   \texttt{\#\#\# Constraints}\\\\
%   \texttt{- The subject may appear, but it must be used in a completely different meaning or context than in the original sentence.}\\\\
%   \texttt{- The passage must contain multiple sentences that expand on the topic with background information, examples, or applications.}\\\\
%   \texttt{- The passage must have no semantic or narrative connection to the original sentence.}\\\\
%   \texttt{- The passage must be complex enough to act as a distractor when answering a question about the original sentence.}\\\\
%   \texttt{- The passage could include any topic such as science, sports, economics, politics, medicine, philosophy, history, or technology.}\\\\
%   \texttt{- The passage must be in the same language as the input sentence.}\\\\
%   \texttt{\#\#\# Output}\\
%   \texttt{Strictly output only the distractor passage and nothing else.}
%   \end{tabular} \\
% \bottomrule
% \end{tabular}%
% }
% \end{center}
% \caption{Prompt template used for generating a moderate-length distractor passage including only the subject but omitting the action and object.}
% \label{tab:prompt_template_case_2}
% \end{table*}

% \begin{table*}[!ht]
% \begin{center}
% \small
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.0}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{p{1.3in}p{5.2in}}
% \toprule
% \textbf{\texttt{Prompt Template for Including Only the Object (Moderate-Length Distractor)}} &
%   \begin{tabular}[c]{@{}p{5.2in}@{}}
%   \texttt{You are given an independent sentence from the bAbI dataset, which follows the Subject -> Action -> Object structure.}\\\\
%   \texttt{\#\#\# Sentence}\\
%   \texttt{\{sentence\}}\\\\
%   \texttt{\#\#\# Task}\\
%   \texttt{Generate a moderate-length passage (100-200 words) that describes the object but never mentions the subject or the action.}\\\\
%   \texttt{\#\#\# Constraints}\\\\
%   \texttt{- The object may appear, but it must be used in a completely different meaning or context than in the original sentence.}\\\\
%   \texttt{- The passage must contain multiple sentences that expand on the topic with background information, examples, or applications.}\\\\
%   \texttt{- The passage must have no semantic or narrative connection to the original sentence.}\\\\
%   \texttt{- The passage must be complex enough to act as a distractor when answering a question about the original sentence.}\\\\
%   \texttt{- The passage could include any topic such as science, sports, economics, politics, medicine, philosophy, history, or technology.}\\\\
%   \texttt{- The passage must be in the same language as the input sentence.}\\\\
%   \texttt{\#\#\# Output}\\
%   \texttt{Strictly output only the distractor passage and nothing else.}
%   \end{tabular} \\
% \bottomrule
% \end{tabular}%
% }
% \end{center}
% \caption{Prompt template used for generating a moderate-length distractor passage including only the object but omitting the subject and action.}
% \label{tab:prompt_template_case_3}
% \end{table*}

% \begin{table*}[!ht]
% \begin{center}
% \small
% \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.0}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{p{1.3in}p{5.2in}}
% \toprule
% \textbf{\texttt{Prompt Template for Including Everything but Unrelated (Moderate-Length Distractor)}} &
%   \begin{tabular}[c]{@{}p{5.2in}@{}}
%   \texttt{You are given an independent sentence from the bAbI dataset, which follows the Subject -> Action -> Object structure.}\\\\
%   \texttt{\#\#\# Sentence}\\
%   \texttt{\{sentence\}}\\\\
%   \texttt{\#\#\# Task}\\
%   \texttt{Generate a moderate-length passage (100-200 words) that includes the subject, action, and object but in a completely different context.}\\\\
%   \texttt{\#\#\# Constraints}\\\\
%   \texttt{- The subject, action, and object must all appear, but they must be used in a completely different meaning or context than in the original sentence.}\\\\
%   \texttt{- The passage must contain multiple sentences that expand on the topic with background information, examples, or applications.}\\\\
%   \texttt{- The passage must have no semantic or narrative connection to the original sentence.}\\\\
%   \texttt{- The passage must be complex enough to act as a distractor when answering a question about the original sentence.}\\\\
%   \texttt{- The passage could include any topic such as science, sports, economics, politics, medicine, philosophy, history, or technology.}\\\\
%   \texttt{- The passage must be in the same language as the input sentence.}\\\\
%   \texttt{\#\#\# Output}\\
%   \texttt{Strictly output only the distractor passage and nothing else.}
%   \end{tabular} \\
% \bottomrule
% \end{tabular}%
% }
% \end{center}
% \caption{Prompt template used for generating a moderate-length distractor passage including everything but unrelated to the original sentence.}
% \label{tab:prompt_template_case_4}
% \end{table*}


==> tables/result_table2.tex <==
% \begin{table*}[t]
% \begin{center}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l|cccccccc}
% \toprule
% \rowcolor[gray]{0.9} \textbf{Language} & \textbf{Method} & \textbf{0} & \textbf{2K} & \textbf{4K} & \textbf{8K} & \textbf{16K} & \textbf{32K} & \textbf{64K} & \textbf{100K} \\ 
% \midrule
% \multirow{6}{*}{\textbf{English}} 
%  & Zeroshot & $0.51$ & $0.50$ & $0.49$ & $0.46$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & Fewshot & $0.62$ & $0.56$ & $0.61$ & $0.47$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & Translation & $0.51$ & $0.51$ & $0.47$ & $0.50$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & CoT & $0.60$ & \underline{$0.75$} & \underline{$0.75$} & $0.75$ & $0.00$ & $0.00$ & $0.34$ & $0.00$ \\
%  & RAG-MpNet & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.43$ & $0.44$ & $0.40$ & $0.44$ \\
%  & RAG-JinaAI & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.47$ & $0.43$ & $0.41$ & $0.40$ \\
% \midrule
% \multirow{6}{*}{\textbf{German}} 
%  & Zeroshot & $0.56$ & $0.53$ & $0.53$ & $0.48$ & $0.00$ & $0.00$ & $0.00$ & $0.41$ \\
%  & Fewshot & $0.59$ & $0.55$ & $0.60$ & $0.57$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & Translation & $0.58$ & $0.53$ & $0.51$ & $0.49$ & $0.00$ & $0.00$ & $0.00$ & $0.41$ \\
%  & CoT & $0.53$ & \underline{$0.79$} & \underline{$0.79$} & $0.71$ & $0.40$ & $0.00$ & $0.00$ & $0.00$ \\
%  & RAG-MpNet & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.50$ & $0.46$ & $0.45$ & $0.43$ \\
%  & RAG-JinaAI & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.23$ & $0.23$ & $0.26$ & $0.24$ \\
% \midrule
% \multirow{6}{*}{\textbf{Spanish}} 
%  & Zeroshot & $0.55$ & $0.49$ & $0.48$ & $0.44$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & Fewshot & $0.57$ & $0.52$ & $0.54$ & $0.60$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & Translation & $0.58$ & $0.47$ & $0.49$ & $0.45$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & CoT & $0.58$ & \underline{$0.77$} & \underline{$0.78$} & $0.73$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & RAG-MpNet & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.48$ & $0.46$ & $0.43$ & $0.45$ \\
%  & RAG-JinaAI & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.39$ & $0.38$ & $0.00$ & $0.40$ \\
% \midrule
% \multirow{6}{*}{\textbf{Chinese}} 
%  & Zeroshot & $0.30$ & $0.26$ & $0.24$ & $0.20$ & $0.21$ & $0.19$ & $0.00$ & $0.25$ \\
%  & Fewshot & $0.41$ & $0.36$ & $0.49$ & $0.50$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & Translation & $0.39$ & $0.27$ & $0.24$ & $0.20$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & CoT & $0.54$ & \underline{$0.62$} & $0.59$ & $0.55$ & $0.00$ & $0.00$ & $0.24$ & $0.00$ \\
%  & RAG-MpNet & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.22$ & $0.21$ & $0.21$ & $0.19$ \\
%  & RAG-JinaAI & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.37$ & $0.37$ & $0.32$ & $0.31$ \\
%  \midrule
% \multirow{6}{*}{\textbf{Chinese}} 
%  & Zeroshot & $0.30$ & $0.26$ & $0.24$ & $0.20$ & $0.21$ & $0.19$ & $0.00$ & $0.25$ \\
%  & Fewshot & $0.41$ & $0.36$ & $0.49$ & $0.50$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & Translation & $0.39$ & $0.27$ & $0.24$ & $0.20$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & CoT & $0.54$ & \underline{$0.62$} & $0.59$ & $0.55$ & $0.00$ & $0.00$ & $0.24$ & $0.00$ \\
%  & RAG-MpNet & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.22$ & $0.21$ & $0.21$ & $0.19$ \\
%  & RAG-JinaAI & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.37$ & $0.37$ & $0.32$ & $0.31$ \\
%  \midrule
% \multirow{6}{*}{\textbf{Chinese}} 
%  & Zeroshot & $0.30$ & $0.26$ & $0.24$ & $0.20$ & $0.21$ & $0.19$ & $0.00$ & $0.25$ \\
%  & Fewshot & $0.41$ & $0.36$ & $0.49$ & $0.50$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & Translation & $0.39$ & $0.27$ & $0.24$ & $0.20$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & CoT & $0.54$ & \underline{$0.62$} & $0.59$ & $0.55$ & $0.00$ & $0.00$ & $0.24$ & $0.00$ \\
%  & RAG-MpNet & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.22$ & $0.21$ & $0.21$ & $0.19$ \\
%  & RAG-JinaAI & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.37$ & $0.37$ & $0.32$ & $0.31$ \\
%  \midrule
% \multirow{6}{*}{\textbf{Chinese}} 
%  & Zeroshot & $0.30$ & $0.26$ & $0.24$ & $0.20$ & $0.21$ & $0.19$ & $0.00$ & $0.25$ \\
%  & Fewshot & $0.41$ & $0.36$ & $0.49$ & $0.50$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & Translation & $0.39$ & $0.27$ & $0.24$ & $0.20$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & CoT & $0.54$ & \underline{$0.62$} & $0.59$ & $0.55$ & $0.00$ & $0.00$ & $0.24$ & $0.00$ \\
%  & RAG-MpNet & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.22$ & $0.21$ & $0.21$ & $0.19$ \\
%  & RAG-JinaAI & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.37$ & $0.37$ & $0.32$ & $0.31$ \\
%  \midrule
% \multirow{6}{*}{\textbf{Chinese}} 
%  & Zeroshot & $0.30$ & $0.26$ & $0.24$ & $0.20$ & $0.21$ & $0.19$ & $0.00$ & $0.25$ \\
%  & Fewshot & $0.41$ & $0.36$ & $0.49$ & $0.50$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & Translation & $0.39$ & $0.27$ & $0.24$ & $0.20$ & $0.00$ & $0.00$ & $0.00$ & $0.00$ \\
%  & CoT & $0.54$ & \underline{$0.62$} & $0.59$ & $0.55$ & $0.00$ & $0.00$ & $0.24$ & $0.00$ \\
%  & RAG-MpNet & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.22$ & $0.21$ & $0.21$ & $0.19$ \\
%  & RAG-JinaAI & $-$ & $0.00$ & $0.00$ & $0.00$ & $0.37$ & $0.37$ & $0.32$ & $0.31$ \\
% \bottomrule
% \end{tabular}%
% }
% \end{center}
% \caption{Performance of various methods across different languages and context lengths. Scores represent accuracy. The highest accuracy within a language is underlined.}
% \label{tab:language_results}
% \end{table*}


% \begin{figure*}[t]
% \includegraphics[width=\textwidth,keepaspectratio,trim={0 0 0 0},clip]{latex/figures/result_table2.pdf}
% \caption{Result Table 2 (monolingual performance across context size)}
% \label{fig:result_table2}
% % \vspace{-0.5mm}
% % \vspace{-5mm}
% \end{figure*}


% \begin{figure*}[t]
% \includegraphics[width=\textwidth,keepaspectratio,trim={0 0 0 0},clip]{latex/figures/result_table2b.pdf}
% \caption{Result Table 2 (monolingual performance across context size)}
% \label{fig:result_table2}
% % \vspace{-0.5mm}
% % \vspace{-5mm}
% \end{figure*}


==> tables/result_table_babi.tex <==
\begin{table*}[!ht]
\begin{center}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Model} & \textbf{en} & \textbf{es} & \textbf{de} & \textbf{zh} & \textbf{vi} & \textbf{hi} & \textbf{ar} \\
\midrule
Meta-Llama-3.1-8B-Instruct & \cellcolor{green!45}0.563 & \cellcolor{green!35}0.523 & \cellcolor{green!30}0.5205 & \cellcolor{green!5}0.245 & \cellcolor{green!10}0.322 & \cellcolor{green!15}0.3305 & \cellcolor{green!0}0 \\
Meta-Llama-3.2-3B-Instruct & \cellcolor{green!40}0.482 & \cellcolor{green!25}0.436 & \cellcolor{green!20}0.4305 & \cellcolor{green!0}0.179 & \cellcolor{green!10}0.34 & \cellcolor{green!10}0.304 & \cellcolor{green!0}0 \\
CohereForAI-aya-23-8B & \cellcolor{green!45}0.5515 & \cellcolor{green!35}0.5265 & \cellcolor{green!35}0.534 & \cellcolor{green!10}0.3025 & \cellcolor{green!20}0.3775 & \cellcolor{green!5}0.2525 & \cellcolor{green!1}0.0105 \\
Mistral-7B-Instruct-v0.2 & \cellcolor{green!45}0.5615 & \cellcolor{green!30}0.511 & \cellcolor{green!30}0.521 & \cellcolor{green!25}0.4465 & \cellcolor{green!20}0.381 & \cellcolor{green!15}0.3585 & \cellcolor{green!40}0.4295 \\
Qwen2-7B-Instruct & \cellcolor{green!50}0.5755 & \cellcolor{green!35}0.522 & \cellcolor{green!30}0.504 & \cellcolor{green!25}0.429 & \cellcolor{green!30}0.46 & \cellcolor{green!15}0.3545 & \cellcolor{green!5}0.131 \\
\midrule
\textbf{Overall} & & & & & & & \\
\midrule
Meta-Llama-3.1-8B-Instruct & \cellcolor{green!50}0.582 & \cellcolor{green!40}0.541 & \cellcolor{green!35}0.532 & \cellcolor{green!5}0.242 & \cellcolor{green!10}0.34 & \cellcolor{green!25}0.377 & \cellcolor{green!0}0 \\
Meta-Llama-3.2-3B-Instruct & \cellcolor{green!35}0.466 & \cellcolor{green!25}0.436 & \cellcolor{green!20}0.43 & \cellcolor{green!0}0.183 & \cellcolor{green!10}0.346 & \cellcolor{green!10}0.296 & \cellcolor{green!0}0 \\
CohereForAI-aya-23-8B & \cellcolor{green!45}0.562 & \cellcolor{green!35}0.536 & \cellcolor{green!45}0.554 & \cellcolor{green!10}0.298 & \cellcolor{green!20}0.399 & \cellcolor{green!10}0.304 & \cellcolor{green!1}0.014 \\
Mistral-7B-Instruct-v0.2 & \cellcolor{green!50}0.603 & \cellcolor{green!45}0.553 & \cellcolor{green!50}0.571 & \cellcolor{green!35}0.501 & \cellcolor{green!25}0.437 & \cellcolor{green!25}0.423 & \cellcolor{green!50}0.482 \\
Qwen2-7B-Instruct & \cellcolor{green!50}0.594 & \cellcolor{green!50}0.56 & \cellcolor{green!40}0.538 & \cellcolor{green!35}0.5 & \cellcolor{green!35}0.492 & \cellcolor{green!15}0.352 & \cellcolor{green!5}0.131 \\
\midrule
\textbf{Context size: 0k} & & & & & & & \\
\midrule
Meta-Llama-3.1-8B-Instruct & \cellcolor{green!40}0.544 & \cellcolor{green!30}0.505 & \cellcolor{green!30}0.509 & \cellcolor{green!5}0.248 & \cellcolor{green!5}0.304 & \cellcolor{green!10}0.284 & \cellcolor{green!0}0 \\
Meta-Llama-3.2-3B-Instruct & \cellcolor{green!40}0.498 & \cellcolor{green!25}0.436 & \cellcolor{green!20}0.431 & \cellcolor{green!0}0.175 & \cellcolor{green!10}0.334 & \cellcolor{green!10}0.312 & \cellcolor{green!0}0 \\
CohereForAI-aya-23-8B & \cellcolor{green!35}0.541 & \cellcolor{green!30}0.517 & \cellcolor{green!30}0.514 & \cellcolor{green!10}0.307 & \cellcolor{green!10}0.356 & \cellcolor{green!5}0.201 & \cellcolor{green!1}0.007 \\
Mistral-7B-Instruct-v0.2 & \cellcolor{green!30}0.52 & \cellcolor{green!20}0.469 & \cellcolor{green!20}0.471 & \cellcolor{green!25}0.392 & \cellcolor{green!10}0.325 & \cellcolor{green!10}0.294 & \cellcolor{green!40}0.377 \\
Qwen2-7B-Instruct & \cellcolor{green!45}0.557 & \cellcolor{green!25}0.484 & \cellcolor{green!20}0.47 & \cellcolor{green!20}0.358 & \cellcolor{green!30}0.428 & \cellcolor{green!15}0.357 & \cellcolor{green!5}0.131 \\
\midrule
\textbf{Context size: 1k} & & & & & & & \\
\bottomrule
\end{tabular}%
}
\end{center}
\caption{Results for monolingual babi task.}
\label{tab:results_multilang}
\end{table*}
